Additive, Near-Additive, and Multiplicative Approximations for APSP in Weighted Undirected Graphs: Trade-offs and Algorithms

We present a $+2\sum_{i=1}^{k+1}{W_i}$-APASP algorithm for dense weighted graphs with runtime $\tilde O\left(n^{2+\frac{1}{3k+2}}\right)$, where $W_{i}$ is the weight of an $i^{th}$ heaviest edge on a shortest path. Dor, Halperin and Zwick [FOCS'96, SICOMP'00] had two algorithms for the commensurate unweighted $+2\cdot\left( k+1\right)$-APASP: $\tilde O\left(n^{2-\frac{1}{k+2}}m^{\frac{1}{k+2}}\right)$ runtime for sparse graphs and $\tilde O\left(n^{2+\frac{1}{3k+2}}\right)$ runtime for dense graphs. Cohen and Zwick [SODA'97, JALG'01] adapted the sparse variant to weighted graphs: $+2\sum_{i=1}^{k+1}{W_i}$-APASP algorithm in the same runtime. We show an algorithm for dense weighted graphs. For nearly additive APASP, we present a $\left(1+\varepsilon,\min{\left\{2W_1,4W_{2}\right\}}\right)$-APASP algorithm with $\tilde O\left(\left(\frac{1}{\varepsilon}\right)^{O\left(1\right)}\cdot n^{2.15135313}\cdot\log W\right)$ runtime. This improves the $\left(1+\varepsilon,2W_1\right)$-APASP of Saha and Ye [SODA'24]. For multiplicative APASP, we show a framework of $\left(\frac{3\ell +4}{\ell + 2}+\varepsilon\right)$-APASP algorithms, reducing the runtime of Akav and Roditty [ESA'21] for dense graphs and generalizing the $\left(2+\varepsilon\right)$-APASP algorithm of Dory et al [SODA'24]. Our base case is a $\left(\frac{7}{3}+\varepsilon\right)$-APASP in $\tilde O\left(\left(\frac{1}{\varepsilon}\right)^{O\left(1\right)}\cdot n^{2.15135313}\cdot \log W\right)$ runtime, improving the $\frac{7}{3}$-APASP algorithm of Baswana and Kavitha [FOCS'06, SICOMP'10] for dense graphs. Finally, we "bypass" an $\tilde \Omega \left(n^\omega\right)$ conditional lower bound by Dor, Halperin, and Zwick for $\alpha$-APASP with $\alpha < 2$, by allowing an additive term (e.g. $\left(\frac{6k+3}{3k+2},\sum_{i=1}^{k+1}W_{i}\right)$-APASP in $\tilde O\left(n^{2+\frac{1}{3k+2}}\right)$ runtime).

==> Algorithms/APASP/ours/1+eps,2W1.tex <==
\begin{algorithm}[t]
\caption{$\paren{1+\varepsilon,2W_{1}}$-APASP$\left(G=\left(V,E,w\right)\right)$}\label{alg:1+eps,2W1}

\textbf{Input:} An undirected non-negative weighted graph $G=\left(V,E,w\right)$ and an arbitrary $\varepsilon>0$.

\textbf{Output:} A  $\paren{1+\varepsilon,2W_{1},4W_{2}}$-APASP. 

\medskip

Let $\beta,\gamma \in \left( 0 , 1 \right)$ to be fixed later

Initialize $d$ as the edges' weights and $\infty$ otherwise

Compute $\Gamma\paren{u,V,n^{\beta}}$ (respectively, $\Gamma\paren{u,V,n^{\beta+\gamma}}$) for all $u\in V$

Compute $S_{1}$ (respectively, $S_{2}$) to be a hitting set to $\bracce{\Gamma\paren{u,V,n^{\beta}} \mid u\in V}$ (respectively, $\Gamma\paren{u,V,n^{\beta+\gamma}}$)

Compute the distances from any $u\in V$ to its pivot $p_{1}\paren{u}$ (respectively, $p_{2}\paren{u}$)

Construct the set of edges $E_{S_{1}}$ (respectively, $E_{S_{2}}$)

Compute MSASP from $S_{2}$ on $G=\paren{V,E,w}$ and update $d$ accordingly

Compute a AMPMM $d_{0}^{2} \star d_{2}^{0}$ and update $d$ accordingly

\For{$i \in <$\hl{$1,0$}$>$}
{
    \For{$s\in  S_{i}$}
    {
        Invoke SSSP from $s$ on $G_{i} \paren{s} = \left( V,E_{ 
 S_{i+1}} \cup \paren{\bracce{s}\times V} \cup H , d \right)$ and update $d$ accordingly
    }
}

\Return $d$


\end{algorithm}\vspace{0mm}

==> Illustrations/Balls/ballexample.tex <==
\begin{figure}[H]
\centering

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp6625860162276211] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.55 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.29 ] (301.45,234.55) .. controls (272.97,209.21) and (270.06,166) .. (294.94,138.04) .. controls (319.82,110.09) and (363.07,107.97) .. (391.55,133.32) .. controls (420.03,158.67) and (422.94,201.87) .. (398.06,229.83) .. controls (373.18,257.78) and (329.93,259.9) .. (301.45,234.55) -- cycle ;
%Straight Lines [id:da9412047664314018] 
\draw    (314.73,189.53) -- (361.23,162.53) ;
%Straight Lines [id:da5938656329561427] 
\draw    (314.73,189.53) -- (358.73,226.2) ;
%Straight Lines [id:da15591646157325867] 
\draw    (358.73,226.2) -- (400.75,264) ;
%Straight Lines [id:da8588636129532099] 
\draw    (358.73,226.2) -- (434.75,226.5) ;
%Straight Lines [id:da3423424168072611] 
\draw    (400.75,264) -- (434.75,226.5) ;
%Straight Lines [id:da7252060609228765] 
\draw    (359.73,225.2) -- (434.25,164) ;
%Straight Lines [id:da8370853051570586] 
\draw    (434.25,164) -- (434.75,222.5) ;
%Straight Lines [id:da23613900566954826] 
\draw    (435.5,165.33) -- (471.75,201) ;
%Straight Lines [id:da18676055033971273] 
\draw    (438.25,162) -- (472.25,147) ;
%Straight Lines [id:da2707706875989797] 
\draw    (472.25,143) -- (472,110.67) ;
%Straight Lines [id:da8302620780031216] 
\draw    (364.23,160.53) -- (468.57,112.87) ;
%Straight Lines [id:da8037223017346966] 
\draw    (365.23,162.53) -- (434.25,163) ;
%Shape: Circle [id:dp40608497322126125] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (357.23,162.53) .. controls (357.23,160.32) and (359.02,158.53) .. (361.23,158.53) .. controls (363.44,158.53) and (365.23,160.32) .. (365.23,162.53) .. controls (365.23,164.74) and (363.44,166.53) .. (361.23,166.53) .. controls (359.02,166.53) and (357.23,164.74) .. (357.23,162.53) -- cycle ;
%Shape: Circle [id:dp26827319251987447] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (354.73,226.2) .. controls (354.73,223.99) and (356.52,222.2) .. (358.73,222.2) .. controls (360.94,222.2) and (362.73,223.99) .. (362.73,226.2) .. controls (362.73,228.41) and (360.94,230.2) .. (358.73,230.2) .. controls (356.52,230.2) and (354.73,228.41) .. (354.73,226.2) -- cycle ;
%Straight Lines [id:da8476855593267647] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (500.25,180) -- (477.58,154.49) ;
\draw [shift={(476.25,153)}, rotate = 48.37] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp9709647852196648] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (310.73,189.53) .. controls (310.73,187.32) and (312.52,185.53) .. (314.73,185.53) .. controls (316.94,185.53) and (318.73,187.32) .. (318.73,189.53) .. controls (318.73,191.74) and (316.94,193.53) .. (314.73,193.53) .. controls (312.52,193.53) and (310.73,191.74) .. (310.73,189.53) -- cycle ;
%Shape: Circle [id:dp5706248374556] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.25,163) .. controls (430.25,160.79) and (432.04,159) .. (434.25,159) .. controls (436.46,159) and (438.25,160.79) .. (438.25,163) .. controls (438.25,165.21) and (436.46,167) .. (434.25,167) .. controls (432.04,167) and (430.25,165.21) .. (430.25,163) -- cycle ;
%Shape: Circle [id:dp6661137907917287] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468,110.67) .. controls (468,108.46) and (469.79,106.67) .. (472,106.67) .. controls (474.21,106.67) and (476,108.46) .. (476,110.67) .. controls (476,112.88) and (474.21,114.67) .. (472,114.67) .. controls (469.79,114.67) and (468,112.88) .. (468,110.67) -- cycle ;
%Shape: Circle [id:dp1158857638153572] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.25,147) .. controls (468.25,144.79) and (470.04,143) .. (472.25,143) .. controls (474.46,143) and (476.25,144.79) .. (476.25,147) .. controls (476.25,149.21) and (474.46,151) .. (472.25,151) .. controls (470.04,151) and (468.25,149.21) .. (468.25,147) -- cycle ;
%Shape: Circle [id:dp7673589811197465] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (467.75,201) .. controls (467.75,198.79) and (469.54,197) .. (471.75,197) .. controls (473.96,197) and (475.75,198.79) .. (475.75,201) .. controls (475.75,203.21) and (473.96,205) .. (471.75,205) .. controls (469.54,205) and (467.75,203.21) .. (467.75,201) -- cycle ;
%Shape: Circle [id:dp5265818224073935] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.75,226.5) .. controls (430.75,224.29) and (432.54,222.5) .. (434.75,222.5) .. controls (436.96,222.5) and (438.75,224.29) .. (438.75,226.5) .. controls (438.75,228.71) and (436.96,230.5) .. (434.75,230.5) .. controls (432.54,230.5) and (430.75,228.71) .. (430.75,226.5) -- cycle ;
%Shape: Circle [id:dp603509841517055] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (396.75,264) .. controls (396.75,261.79) and (398.54,260) .. (400.75,260) .. controls (402.96,260) and (404.75,261.79) .. (404.75,264) .. controls (404.75,266.21) and (402.96,268) .. (400.75,268) .. controls (398.54,268) and (396.75,266.21) .. (396.75,264) -- cycle ;

% Text Node
\draw (383.42,264.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (339.92,226.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (441.83,219.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (418,144) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (479.08,196.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{1}$};
% Text Node
\draw (479.08,107.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{3}$};
% Text Node
\draw (479.25,142.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{2}$};
% Text Node
\draw (357.25,169.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (394,213) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (473.83,121.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.5,163.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (373.33,246.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 2$};
% Text Node
\draw (327,207.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 2$};
% Text Node
\draw (397,193.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 3$};
% Text Node
\draw (328.5,163.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 3$};
% Text Node
\draw (424.33,191) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 9$};
% Text Node
\draw (452,156.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (446.5,185.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (412.17,121.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (416.83,244.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (507.57,185.27) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{17.59pt}\setlength\topsep{0pt}
\textcolor[rgb]{0.29,0.56,0.89}{$\displaystyle p_{S}( u)$}
\end{minipage}};
% Text Node
\draw (295.75,190.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (307.47,127.01) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 45; green, 127; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle ball( u,A,S)$};


\end{tikzpicture}




\caption{\label{fig:ballexample} The ball $ball \left(u,A,S\right)$, where $A=\left\{ a_1,a_2,a_3\right\}$ and $S=\left\{s_1,s_2,s_3\right\}$. The pivot for $u$ is $p\left(u\right) = s_2$ with $\delta\left(u,S\right) = 5$.}
\end{figure}\vspace{-4mm}

==> Illustrations/Balls/inneredgesexample.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da87840787155437] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (315.01,190.03) -- (361.51,163.03) ;
%Straight Lines [id:da052344792013143016] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (315.01,190.03) -- (359.01,226.7) ;
%Straight Lines [id:da704512876406874] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (359.01,226.7) -- (401.03,264.5) ;
%Straight Lines [id:da2529965611042688] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (359.01,226.7) -- (435.03,227) ;
%Straight Lines [id:da038558601052662844] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (401.03,264.5) -- (435.03,227) ;
%Straight Lines [id:da1453158167020543] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (360.01,225.7) -- (434.53,164.5) ;
%Straight Lines [id:da8496894787108054] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (434.53,164.5) -- (435.03,223) ;
%Straight Lines [id:da15583751877941343] 
\draw    (435.78,165.83) -- (472.03,201.5) ;
%Straight Lines [id:da6954206584025682] 
\draw    (438.53,162.5) -- (472.53,147.5) ;
%Straight Lines [id:da9064565291303313] 
\draw    (472.53,143.5) -- (472.28,111.17) ;
%Straight Lines [id:da53256747981667] 
\draw    (364.51,161.03) -- (468.85,113.37) ;
%Straight Lines [id:da35419788722237744] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (365.51,163.03) -- (434.53,163.5) ;
%Shape: Circle [id:dp31720811305789964] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (357.51,163.03) .. controls (357.51,160.82) and (359.3,159.03) .. (361.51,159.03) .. controls (363.72,159.03) and (365.51,160.82) .. (365.51,163.03) .. controls (365.51,165.24) and (363.72,167.03) .. (361.51,167.03) .. controls (359.3,167.03) and (357.51,165.24) .. (357.51,163.03) -- cycle ;
%Shape: Circle [id:dp5265937509664673] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (355.01,226.7) .. controls (355.01,224.49) and (356.8,222.7) .. (359.01,222.7) .. controls (361.22,222.7) and (363.01,224.49) .. (363.01,226.7) .. controls (363.01,228.91) and (361.22,230.7) .. (359.01,230.7) .. controls (356.8,230.7) and (355.01,228.91) .. (355.01,226.7) -- cycle ;
%Shape: Circle [id:dp24609937249348568] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (311.01,190.03) .. controls (311.01,187.82) and (312.8,186.03) .. (315.01,186.03) .. controls (317.22,186.03) and (319.01,187.82) .. (319.01,190.03) .. controls (319.01,192.24) and (317.22,194.03) .. (315.01,194.03) .. controls (312.8,194.03) and (311.01,192.24) .. (311.01,190.03) -- cycle ;
%Shape: Circle [id:dp9874523059430802] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.53,163.5) .. controls (430.53,161.29) and (432.32,159.5) .. (434.53,159.5) .. controls (436.74,159.5) and (438.53,161.29) .. (438.53,163.5) .. controls (438.53,165.71) and (436.74,167.5) .. (434.53,167.5) .. controls (432.32,167.5) and (430.53,165.71) .. (430.53,163.5) -- cycle ;
%Shape: Circle [id:dp8586237542464736] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.28,111.17) .. controls (468.28,108.96) and (470.07,107.17) .. (472.28,107.17) .. controls (474.49,107.17) and (476.28,108.96) .. (476.28,111.17) .. controls (476.28,113.38) and (474.49,115.17) .. (472.28,115.17) .. controls (470.07,115.17) and (468.28,113.38) .. (468.28,111.17) -- cycle ;
%Shape: Circle [id:dp8552923192966435] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.53,147.5) .. controls (468.53,145.29) and (470.32,143.5) .. (472.53,143.5) .. controls (474.74,143.5) and (476.53,145.29) .. (476.53,147.5) .. controls (476.53,149.71) and (474.74,151.5) .. (472.53,151.5) .. controls (470.32,151.5) and (468.53,149.71) .. (468.53,147.5) -- cycle ;
%Shape: Circle [id:dp6801603655991799] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.03,201.5) .. controls (468.03,199.29) and (469.82,197.5) .. (472.03,197.5) .. controls (474.24,197.5) and (476.03,199.29) .. (476.03,201.5) .. controls (476.03,203.71) and (474.24,205.5) .. (472.03,205.5) .. controls (469.82,205.5) and (468.03,203.71) .. (468.03,201.5) -- cycle ;
%Shape: Circle [id:dp7631537577629186] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (431.03,227) .. controls (431.03,224.79) and (432.82,223) .. (435.03,223) .. controls (437.24,223) and (439.03,224.79) .. (439.03,227) .. controls (439.03,229.21) and (437.24,231) .. (435.03,231) .. controls (432.82,231) and (431.03,229.21) .. (431.03,227) -- cycle ;
%Shape: Circle [id:dp4241349705641584] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (397.03,264.5) .. controls (397.03,262.29) and (398.82,260.5) .. (401.03,260.5) .. controls (403.24,260.5) and (405.03,262.29) .. (405.03,264.5) .. controls (405.03,266.71) and (403.24,268.5) .. (401.03,268.5) .. controls (398.82,268.5) and (397.03,266.71) .. (397.03,264.5) -- cycle ;

% Text Node
\draw (383.7,265) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (340.2,227) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (442.11,219.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (418.28,144.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (479.36,197) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{1}$};
% Text Node
\draw (479.36,107.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{3}$};
% Text Node
\draw (479.53,142.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{2}$};
% Text Node
\draw (357.53,170) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (394.28,213.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 1$};
% Text Node
\draw (474.11,121.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.78,164) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 1$};
% Text Node
\draw (373.61,246.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 2$};
% Text Node
\draw (327.28,207.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 2$};
% Text Node
\draw (397.28,193.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 3$};
% Text Node
\draw (328.78,164.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 3$};
% Text Node
\draw (424.61,191.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 9$};
% Text Node
\draw (452.28,156.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (446.78,185.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (412.45,122.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (417.11,245) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 4$};
% Text Node
\draw (296.03,190.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};


\end{tikzpicture}

\caption{\label{fig:inneredgesexample} The inner-edges $E_{S}$ of all vertices $V$, in relation to $S$.}
\end{figure}

==> Tables/APASP/known_res_unweighted.tex <==

\begin{table}[H]%icalp:H
  \begin{center}
\small\addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{|c|c|c|} %1st col was: p{3cm}
      \hline
      \textbf{\small Approximation} & \textbf{\small Combinatorial}  & \textbf{\small Algebraic} \\
      \hhline{|=|=|=|}
      &&\\ [-1em]
      $1$&  -- & $n^{\omega} $  \cite{Seidel1995} \\ 
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$+2$}& \multirow{2}{*}{$\mmin{n^{\frac{7}{3}},n^{\frac{3}{2}}m^{\frac{1}{2}}}$ \cite{DorHalZwi2000}}  & $n^{2} t^{\frac{1}{2}}+MPCRBD(n,\frac{n}{t})$ \multirow{2}{*}{\qquad\cite{DenKirVicVasZho2022}}\\
      &&$\approx n^{2.2867}$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\left(1+\varepsilon,2\right)$}& \multirow{2}{*}{--} & $n^{2+\frac{1-r}{2}}+\frac{1}{\varepsilon}n^{\omega\left(r\right)}$ \multirow{2}{*}{\qquad\cite{DorForKirNazVasVos2023}}\\ 
      & & $\approx \frac{1}{\varepsilon}\cdot n^{2.15135313}$ \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\left(1+\varepsilon,4\right)$}&  \multirow{2}{*}{--} & $n^{2+\frac{1-r}{3}}+\frac{1}{\varepsilon}n^{\omega\left(r\right)}$ \multirow{2}{*}{\qquad \cite{DorForKirNazVasVos2023}}\\
      & & $\approx \frac{1}{\varepsilon}\cdot n^{2.1185119}$ \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\left(1+\varepsilon,6\right)$}&  \multirow{2}{*}{--} & $n^{2+\frac{1-r}{4}}+\frac{1}{\varepsilon}n^{\omega\left(r\right)}$ \multirow{2}{*}{\qquad\cite{DorForKirNazVasVos2023}}\\ 
      &&$\approx \frac{1}{\varepsilon}\cdot n^{2.09778592}$ \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\left(1+\varepsilon,8\right)$}&  \multirow{2}{*}{--} & $n^{2+\frac{1-r}{5}}+\frac{1}{\varepsilon}n^{\omega\left(r\right)}$ \multirow{2}{*}{\qquad \cite{DorForKirNazVasVos2023}} \\
      && $\approx \frac{1}{\varepsilon}\cdot n^{2.08346083}$ \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $+2\cdot\left(k+1\right)$& $\mmin{n^{2+\frac{1}{3k+2}},n^{2-\frac{1}{k+2}}m^{\frac{1}{k+2}}}$ \cite{DorHalZwi2000} & =\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$2$}& \multirow{2}{*}{$n^{\frac{9}{4}}$\cite{DorForKirNazVasVos2023, Roditty2023}} & $n^{\frac{5}{2}-r} +n^{\omega\left(r\right)}$ \multirow{2}{*}{\qquad \cite{DorForKirNazVasVos2023}}\\
      &&$\approx n^{2.03106234}$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\frac{7}{3}$}& \multirow{2}{*}{$n^{2}$\cite{SahYe2023} }& \multirow{2}{*}{--}\\
      &&\\
      \hline
    \end{tabular}
    \caption{Known combinatorial and algebraic APASP runtimes for unweighted graphs. }~\label{tab:known_unweighted}
  \end{center}
\end{table} 

==> Tables/APASP/known_res_weighted.tex <==
\begin{table}[H]%icalp:H
  \begin{center}
    
\small\addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{|c|c|c|} %1st col was: p{3cm}
      \hline
      \textbf{\small Approximation} & \textbf{\small Combinatorial}  & \textbf{\small Algebraic} \\
      \hhline{|=|=|=|}
      &&\\ [-1em]
      $1+\varepsilon$& -- & $\frac{1}{\varepsilon} \cdot n^{\omega} \cdot \log\frac{n}{\varepsilon} $ \cite{BriKunWun2019}  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $+2W_{2}$& $n^{\frac{3}{2}} m ^{\frac{1}{2}} $ \cite{CohZwi1997} &  - \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $+\mmin{2W_{1},4W_{2}}$& $n^{\frac{7}{3}} $ \cite{CohZwi1997} &  - \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\left(1+\varepsilon,2W_{1}\right)$}& \multirow{2}{*}{--}  &  $\frac{1}{\varepsilon}\cdot n^{\omega\paren{1,1-x,1}}\cdot \log W + n^{2+\frac{x}{2}}$ \multirow{2}{*}{\qquad\cite{SahYe2023}} \\
      &  & $\approx \frac{1}{\varepsilon}\cdot n^{2.15135313}\cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $+2\msum{W_{i}}{i=1}{k+1} $& $n^{2-\frac{1}{k+2}}m^{\frac{1}{k+2}}$ \cite{CohZwi1997} &  --  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\left(1+\varepsilon,2\msum{W_{i}}{i=1}{k+1}\right)$& --  &  $\frac{1}{\varepsilon}\cdot n^{\omega\paren{1-\frac{k}{k+2}\cdot x,1-x,1-\frac{k-1}{k+2}\cdot x}}\cdot \log W + n^{2+\frac{x}{k+2}}$ \cite{SahYe2023} \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $2$& $n^{\frac{1}{2}}m+n^2$ \cite{BasKav2010,AkaRod2021} &  --  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$2+\varepsilon$}& \multirow{2}{*}{--} &  $n^{1-r}m + \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)}n^{\omega\left(r\right)}\cdot \log W $ \multirow{2}{*}{\qquad\cite{DorForKirNazVasVos2023}}  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.21235201}\cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\left(2,W_{1}\right)$& $n^2$ \cite{BasKav2010,BerKas2007} &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\frac{7}{3}$& $nm^{\frac{2}{3}}+n^2$ \cite{BasKav2010,AkaRod2021} &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\frac{5}{2}$& $n^{\frac{5}{4}}m^{\frac{1}{2}}+n^{2}$ \cite{Kavitha2012,AkaRod2021} &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\frac{3\ell+4}{\ell+2}$& $n^{2-\frac{3}{\ell+2}}m^{\frac{2}{\ell+2}}+n^2$ \cite{AkaRod2021} & --  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$3$}& \multirow{2}{*}{$n^{2}$ \cite{CohZwi1997,BasKav2010}}  & \multirow{2}{*}{--}  \\
      &&\\
      \hline
    \end{tabular}
    \caption{Known combinatorial and algebraic APASP runtimes for weighted graphs.}~\label{tab:known_weighted}
  \end{center}
\end{table} 

==> Tables/APASP/our_res_equiv_n1over3k+2.tex <==
\begin{table}[H]%icalp:H
  \begin{center}
    
\small\addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{|c|c|} %1st col was: p{3cm}
      \hline
      \textbf{\small Approximation} & \textbf{\small Combinatorial} \\
      \hhline{|=|=|}
      &\\ [-1em]
      $+2\msum{W_{i}}{i=1}{k+1} $& $n^{2+\frac{1}{3k+2}}$    \\
      &\\ [-1em]
      \hline
      &\\ [-1em]
      $\paren{\frac{6k+3}{3k+2},\msum{W_{i}}{i=1}{k+1}} $& $n^{2+\frac{1}{3k+2}}$  \\
      &\\ [-1em]
      \hline
      &\\ [-1em]      $\paren{\frac{\paren{9k+4}\cdot\alpha+\paren{3k+2}\cdot\beta}{\paren{\alpha+\beta}\cdot\paren{3k+2}},\frac{2\beta}{\alpha+\beta}\msum{W_{i}}{i=1}{k+1}}$& $n^{2+\frac{1}{3k+2}}$  \\
      &\\ [-1em]
      \hline
      &\\ [-1em]
      $\frac{9k+4}{3k+2}$& $\leq n^{2+\frac{1}{3k+2}}$  \cite{AkaRod2021}  \\
      &\\ 
      \hline
    \end{tabular}
    \caption{Runtime equivalence for $\tilde O\paren{n^{2+\frac{1}{3k+2}}}$.}~\label{tab:our_res_equiv_n1over3k+2}
  \end{center}
\end{table} 

==> Tables/APASP/our_res_equiv_n7over3.tex <==
\begin{table}[H]
  \begin{center}
    
\small\addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{|c|c|c|} %1st col was: p{3cm}
      \hline
      \textbf{\small Approximation} & \textbf{\small Combinatorial}  & \textbf{\small Algebraic} \\
      \hhline{|=|=|=|}
      &&\\ [-1em]
      $+2\mmin{2W_{1},4W_{2}} $& $n^{\frac{7}{3}}$ \cite{CohZwi1997}  &  --  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\paren{\frac{3}{2},W_{1}+\frac{W_{2}}{2}} $& $n^{\frac{7}{3}}$ &  --  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\left(\frac{3}{2},\frac{5W_{1}}{4}\right)$& $n^\frac{7}{3}$  &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\left(2,\frac{W_{1}}{2}\right)$& $n^\frac{7}{3}$  &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\left(2,W_{2}\right)$& $n^\frac{7}{3}$  &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\left(\frac{11}{5},\frac{2W_{2}}{5}\right)$& $n^\frac{7}{3}$  &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\left(\frac{9}{4},\frac{W_{2}}{2}\right)$& $n^\frac{7}{3}$  &  -- \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\frac{7}{3} $& $\leq n^{\frac{7}{3}}$ \cite{BasKav2010}  &  --  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\left(1+\varepsilon,\mmin{2W_{1},4W_{2}}\right)$}& \multirow{2}{*}{--}  &  $n^{2+\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      &  & $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\paren{\frac{3}{2}+\varepsilon,W_{1}+\frac{W_{2}}{2}}$}& \multirow{2}{*}{--} &  $n^{2+\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\paren{\frac{3}{2}+\varepsilon,\frac{5W_{1}}{4}}$}& \multirow{2}{*}{--} &  $n^{2+\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\paren{2+\varepsilon,\frac{W_{1}}{2}}$}& \multirow{2}{*}{--} &  $n^{2+\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\paren{2+\varepsilon,W_{2}}$}& \multirow{2}{*}{--} &  $n^{2+\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\paren{\frac{11}{5}+\varepsilon,\frac{2W_{2}}{5}}$}& \multirow{2}{*}{--} &  $n^{2+\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\paren{\frac{9}{4}+\varepsilon,\frac{W_{2}}{2}}$}& \multirow{2}{*}{--} &  $n^{2+\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\frac{7}{3}+\varepsilon$}& \multirow{2}{*}{--} &  $mn^{\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
    \end{tabular}
    \caption{Runtime equivalence for $\tilde O\paren{n^{\frac{7}{3}}}$ or $\tilde O_{\varepsilon,W} \paren{n^{2.15135313}}$.}~\label{tab:our_res_equiv_n7over3}
  \end{center}
\end{table} 

==> Tables/APASP/our_res_weighted.tex <==
\begin{table}[H]%icalp:H
  \begin{center}
    
\small\addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{|c|c|c|} %1st col was: p{3cm}
      \hline
      \textbf{\small Approximation} & \textbf{\small Combinatorial}  & \textbf{\small Algebraic} \\
      \hhline{|=|=|=|}
      &&\\ [-1em]
      $+2\msum{W_{i}}{i=1}{k+1} $& $n^{2+\frac{1}{3k+2}}$  &  --  \\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\left(1+\varepsilon,\mmin{2W_{1},4W_{2}}\right)$}& \multirow{2}{*}{--}  &  $mn^{\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      &  & $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      \multirow{2}{*}{$\frac{7}{3}+\varepsilon$}& \multirow{2}{*}{--} &  $mn^{\beta} + n^{2+\gamma} +\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma\right)} \cdot  \log W$  \\
      && $\approx \left(\frac{1}{\varepsilon}\right)^{O\left(1\right)} \cdot n^{2.15135313} \cdot \log W$\\
      &&\\ [-1em]
      \hline
      &&\\ [-1em]
      $\frac{3\ell+4}{\ell+2}+\varepsilon$& -- & $mn^{\beta}+\msum{n^{2+\gamma_{i}}}{i=1}{\ell}+\left(\frac{1}{\varepsilon} \right)^{O\left(1\right)} \cdot n^{\omega\left(1-\beta-\gamma_{1}-\ldots-\gamma_{\ell}\right)} \cdot  \log W $  \\
      \hline
    \end{tabular}
    \caption{Our results for combinatorial and algebraic APASP for weighted graphs.}~\label{tab:our_weighted}
  \end{center}
\end{table} 

==> Temporary/1+eps,2W1.tex <==
\section{Near-additive $\paren{1+\varepsilon,2W_{1}}$-APASP}~\label{1+eps,2W1}

\input{\apaspAlgoPath ours/1+eps,2W1}

In \cite{DorForKirNazVasVos2023}, the authors described an algorithm that combines an algorithm for $2$-APASP  \cite{BasKav2010} and a $\paren{1+\varepsilon}$-MSASP invocation \cite{ElkNei2020} (see \thmref{1pluseps_msasp} and \thmref{1pluseps_minplus}) to compute a $\paren{2+\varepsilon}$-APASP for any $\varepsilon>0$. Our simplified approach allows us to consider a similar approach. We adjust \algref{+2W1}, \hl{highlighting} the changes:
\begin{enumerate}
    \item Instead of conducting multiple SSSP invocation from all $s\in S_{2}$, we perform a single\footnote{This is a single MSASP invocation as the sources  share the entire set of edges.} $\paren{1+\varepsilon}$-MSASP from $S_{2}$ by applying \thmref{1pluseps_msasp}, 
    \item Instead of taking into account the set of edges $S_{2}\times S_{0}$  when invoking SSSP from any $s\in S_{0}\cup S_{1}$, we perform an AMPMM of two rectangular matrices $d_{0}^{2} \times d_{2}^{0}$ by applying \thmref{1pluseps_minplus}, where $d_{i}^{j}$ is a rectangular matrix containing all estimated distances computed within $d$, its rows narrowed down to include only the vertices of $S_{i}$ and its columns those of $S_{j}$.
\end{enumerate}

We revisit the runtime and correctness proofs of \thmref{+2W1}. The proofs of \lemref{+2W1_case_notb} and \lemref{+2W1_case_b} remain as is. The case analysis presented in \figref{+2W1_casetree} remains the same, apart from \lemref{1+eps,2W1_case_nota} that replaces \lemref{+2W1_case_nota}.

\begin{lemma}~\label{lem:1+eps,2W1_case_nota} 
   If \notcase{a} holds then $d\bracke{u,v} \leq \paren{1+\varepsilon}\cdot\delta\paren{u,v}+2w\paren{a,b}$.
\end{lemma}
\begin{proof}

    Recall that we invoke MSASP from  $S_{2}$, utilizing the entire edge set $E$. We have an estimate: $d\bracke{p_{2}\paren{x},v} \leq \paren{1+\varepsilon}\cdot \delta\paren{p_2\paren{x},v}$ and $d\bracke{u,p_{2}\paren{x}} \leq \paren{1+\varepsilon}\cdot \delta\paren{u,p_2\paren{x}}$. Therefore, when we invoke AMPMM on $d_0^2\star d_2^0$:

    \begin{alignat*}{3}
        d\bracke{u,v} &\leq \textubrace{\paren{1+\varepsilon}\cdot\paren{d\bracke{u,p_{2}\paren{x}}+  d\bracke{p_{2}\paren{x},v}}}{AMPMM on $d_0^2\star d_2^0$}
                && = \textubrace{ \paren{1+\varepsilon}\cdot \paren{\paren{1+\varepsilon}\cdot\delta\paren{u,p_{2}\paren{x}} + \paren{1+\varepsilon}\cdot\delta\paren{p_{2}\paren{x},v}}}{Our preceding discussion}\\ 
                & \leq \textubrace{ \paren{1+\varepsilon}^2\cdot\paren{\delta\paren{u,x } + 2 \cdot \delta\paren{x,p_{2}\paren{x}} + \delta\paren{x,v}}}{Triangle inequality}
               &&= \textubrace{ \paren{1+2\varepsilon+\varepsilon^{2}}\cdot \paren{\delta\paren{u,v } + 2 \cdot \delta\paren{x,p_{2}\paren{x}}}}{$u\squiggly x \squiggly v$ is a shortest path}\\
               & \leq \textubrace{ \paren{1+2\varepsilon +\varepsilon^{2}}\cdot\delta\paren{u,v } +  \paren{2+4\varepsilon +2\varepsilon^{2}}\cdot w\paren{a,b}}{By \notcase{a}} && \leq \textubrace{ \paren{1+6\varepsilon +3\varepsilon^{2}}\cdot\delta\paren{u,v } + 2 \cdot w\paren{a,b}}{As $w\paren{a,b}\leq\delta\paren{u,v}$}
        \end{alignat*}
By selecting  $\varepsilon' = 1+6\varepsilon +3\varepsilon^{2}$, we complete the proof.
\end{proof}

\begin{theorem}~\label{thm:1+eps,2W1} 
    Let $W\in \mathbb{N}$, $\varepsilon>0$ and $G=\left(V,E,w\right)$ be a weighted graph, whose weights are from $\left\{ 0,1,\ldots, W\right\}\cup\left\{\infty\right\}$. \algref{1+eps,2W1} computes a $\paren{1+\varepsilon,2W_{1}}$-APASP in $\tilde O\paren{n^{1+2\beta+2\gamma}+n^{2+\beta} + n^{2+\gamma} + \paren{\frac{1}{\varepsilon}}^{O\paren{1}}\cdot n^{\omega\paren{1-\beta-\gamma}}\cdot \log W}$ time.
\end{theorem}
\begin{proof}

    The correctness follows from \lemref{1+eps,2W1_case_nota}, \lemref{+2W1_case_notb} and \lemref{+2W1_case_b}. As for the runtime, we consider the changes made by the highlighted parts.  Recall that $\abs{S_{2}} \in \tilde O \paren{n^{1-\beta-\gamma}}$. Hence, by \thmref{1pluseps_msasp}, the MSASP invocation requires $\tilde O \paren{m^{1+o\paren{1}} + \paren{ \frac{1}{\varepsilon} }^{O\paren{1}} \cdot n^{\omega\paren{1-\beta-\gamma}} \cdot  \log W}$. By \thmref{1pluseps_minplus}, the AMPMM of $d_{0}^{2} \times d_{2}^{0}$ requires $\tilde O \paren{\frac{1}{\varepsilon} \cdot n^{ \omega\paren{1-\beta-\gamma}} \cdot \log W }$, as $\abs{S_{0}}=\abs{V}= n$. 

    Implementing the SSSP invocations from $S_{1}$ and $S_{1}$ by Dijkstra, we get additional $\tilde O \paren{\abs{S_{0}}\cdot \abs{E_{S_{1}}} + \abs{S_{1}}\cdot \abs{E_{S_{2}}}}  = \tilde O \paren{n^{2+\beta} + n^{2+\gamma}}$ time, as we no longer consider the edges $S_{2}\times S_{0}$. The remaining parts are exactly as is in \thmref{+2W1}, requiring $\tilde O \paren{n^{1+2\beta+2\gamma}}$ time. 
\end{proof}

We can  \cite{complexityBalancer} select $\beta=\gamma \approx 0.15135313$. Hence:

\begin{conclusion}
   \algref{1+eps,2W1} computes a $\paren{1+\varepsilon,2W_{1}}$-APASP in $\tilde O\paren{\paren{\frac{1}{\varepsilon}}^{O\paren{1}}\cdot n^{2.15135313}\cdot \log W}$ time, for an arbitrary $\varepsilon>0$ and weights of the set $\left\{ 0,1,\ldots, W\right\}\cup\left\{\infty\right\} $.
\end{conclusion}
